How Gender Debiasing Affects Internal Model Representations, and Why It Matters

Common studies of gender bias in NLP focus either on extrinsic bias measured by model performance on a downstream task or on intrinsic bias found in models' internal representations. However, the relationship between extrinsic and intrinsic bias is relatively unknown. In this work, we illuminate this relationship by measuring both quantities together: we debias a model during downstream fine-tuning, which reduces extrinsic bias, and measure the effect on intrinsic bias, which is operationalized as bias extractability with information-theoretic probing. Through experiments on two tasks and multiple bias metrics, we show that our intrinsic bias metric is a better indicator of debiasing than (a contextual adaptation of) the standard WEAT metric, and can also expose cases of superficial debiasing. Our framework provides a comprehensive perspective on bias in NLP models, which can be applied to deploy NLP systems in a more informed manner. Our code and model checkpoints are publicly available.

==> tables/CEAT.tex <==
\begin{table*}[h]
\centering

\subfloat[Occupation classification. The difference between a debiased model and a non-debiased model is insignificnat ($p>0.4$ as tested by Pitman's permutation test)]{
\quad
\begin{tabular}{cc}
\toprule
\textbf{Debiasing} & \textbf{CES} \\
\textbf{Strategy} &  \\
\hline
Pre-trained &  0.488\\
\hline
None & 0.224 \\
\hline
Oversampling & 0.292 \\
\hline
Subsampling & 0.225 \\
\hline
Scrubbing & 0.231 \\
\bottomrule
\end{tabular}
\quad
}%
\hspace{5em}
\subfloat[Coreference Resolution: The differences between debiased models and non-debiased model is significant ($p<0.05$ as tested by Pitman's permutation test)]{
\quad
\begin{tabular}{cc}
\toprule
\textbf{Debiasing} & \textbf{CES} \\
\textbf{Strategy} &  \\
\hline
Pre-trained &  0.488 \\
\hline
None & 0.353 \\
\hline
Anonymization & 0.302 \\
\hline
CA & 0.269 \\
\hline
Anonymization + CA & 0.252 \\
\bottomrule
\end{tabular}
\quad
}

\caption{combined effect size (CES) as measured on a RoBERTa model. The numbers as presented for the fine-tuned models are averaged over 10 models, and we kept only values where $p<0.05$, which was 90\% and 95\% of the values for occupation classification and coreference resolution, respectively.}
\end{table*}
\label{tbl:ceat}


==> tables/before-after-comparison-bios.tex <==
\begin{table*}[h]
\adjustbox{max width=\textwidth}{%
\centering
\begin{tabular}{lrrrrrrrrrr}
\toprule
&   &   & \multicolumn{8}{c}{\textbf{Extrinsic}} \\
\cmidrule(lr){4-11}
\multirow{2}{*}{\textbf{\shortstack[l]{Debiasing \\ Strategy}}}  & \multicolumn{2}{c}{\textbf{Intrinsic}} & \multicolumn{4}{c}{\textbf{Before}} & \multicolumn{4}{c}{\textbf{After}} \Bstrut \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11} \Bstrut
   & Compression & CEAT &  TPR (P)  &  FPR (S) &  Sep &  Suff  & TPR (P)   &  FPR (S) &  Sep &  Suff \Bstrut\Tstrut\\
\midrule
Random & 5.61* & 0.12$\dagger$ & - & - & - & - & - & - & - & - \Tstrut\\
Pre-trained & 10.12 & 0.49* & - & - & - & - & - & - & - & - \\
None             & 4.12 & 0.22 & 0.76 & 0.08 & 0.33 & 9.45 & 0.78 & 0.073 & 0.33 & 9.70 \\
Oversampling     & 8.52* &  0.29 & 0.73 & 0.09* & 0.31 & 8.32* & 0.81* & 0.068* & 0.33 & 10.91* \\
Subsampling      & 3.57 & 0.22 & \textbf{0.32}* & \textbf{0.03}* & \textbf{0.20}* & \textbf{1.22}* & \textbf{8.37}* & 0.08* & 0.30* & 1.32* \\
Scrubbing        & \textbf{1.70}* & 0.23 & 0.70* & 0.06* & 0.30 & 4.93* &  0.71* & \textbf{0.06}* & \textbf{2.56}* & \textbf{0.81}* \\
\bottomrule
\end{tabular}
}
\caption{Occupation classification: Comparison of intrinsic and extrinsic metrics before and after retraining of classification layer, over 10 seeds per fine-tuned model and per re-trained classification model. * marks significant reduction or increase in bias ($p < 0.05$ on Pitman's permutation test), compared to the non-debiased model (debiasing strategy None). The lowest bias score in each column is marked with \textbf{bold}. P = Pearson; S = Sum. $\dagger$ was computed only on 3 out of 10 tests for which the p value was $< 0.05$.}
    \label{tbl:before-after-bios}
    \vspace{-10pt}
\end{table*}

==> tables/before-after-comparison-coref.tex <==
\begin{table*}[h]
\adjustbox{max width=\textwidth}{%
\centering
\begin{tabular}{lrrrrrrrrrr}
\toprule
&   &   & \multicolumn{8}{c}{\textbf{Extrinsic}} \\
\cmidrule(lr){4-11}
\multirow{2}{*}{\textbf{\shortstack[l]{Debiasing \\ Strategy}}} & \multicolumn{2}{c}{\textbf{Intrinsic}}  & \multicolumn{4}{c}{\textbf{Before}} & \multicolumn{4}{c}{\textbf{After}} \Bstrut \\
\cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}
   & Compression & CEAT &  F1 diff  & FPR (S) &  Sep &  Suff  & F1 diff &  FPR (S) &  Sep &  Suff \Bstrut\Tstrut\\
\midrule
Random      & 0.83*            & -      & -              & -               & -                      & - & - & - & - & - \Tstrut\\
Pre-trained & 0.96            & 0.49*   & -              & -               & -                      & - & - & - & - & - \\
None        & 1.98            & 0.35  & 6.63           & 0.12            & 1.25                   & 8.69 & 6.07 & 0.11 & 1.19 & 7.35 \\
Anon        & 2.07*           & 0.31*  & 7.26           & 0.13            &  1.34                  & 8.82 &  7.42* &  0.13* & 1.34* & 8.66* \\
CA          &  \textbf{1.50}* & 0.27*   & \textbf{2.30}* & 0.05*           &  \textbf{0.54}*        & 1.67 * & 3.67* & 0.06* & 0.67* & 2.40* \\
Anon + CA   & 1.54*           & \textbf{0.25}*  & 2.42*          & \textbf{0.049}* & 0.56* & \textbf{1.56}* &    \textbf{2.86}* & \textbf{0.05}*  & \textbf{0.59}* &  \textbf{1.65}* \\
\bottomrule
\end{tabular}
}
    \caption{Coreference resolution: Comparison of intrinsic and extrinsic metrics before and after retraining of classification layer, over 10 seeds per fine-tuned model and 5 seeds per retrained classification model. * Marks significant reduction or increase in bias ($p < 0.05$ on Pitman's permutation test), compared to the non-debiased model (debiasing strategy None). The lowest bias score in each column is in \textbf{bold}. P = Pearson; S = Sum.}
    \label{tbl:before-after-coref}
    \vspace{-10pt}
\end{table*}
